Learned Hardware/Software Co-Design of Neural Accelerators

The use of deep learning has grown at an exponential rate, giving rise to numerous specialized hardware and software systems for deep learning. Because the design space of deep learning software stacks and hardware accelerators is diverse and vast, prior work considers software optimizations separately from hardware architectures, effectively reducing the search space. Unfortunately, this bifurcated approach means that many profitable design points are never explored. This paper instead casts the problem as hardware/software co-design, with the goal of automatically identifying desirable points in the joint design space. The key to our solution is a new constrained Bayesian optimization framework that avoids invalid solutions by exploiting the highly constrained features of this design space, which are semi-continuous/semi-discrete. We evaluate our optimization framework by applying it to a variety of neural models, improving the energy-delay product by 18% (ResNet) and 40% (DQN) over hand-tuned state-of-the-art systems, as well as demonstrating strong results on other neural network architectures, such as MLPs and Transformers.

==> ICLR'21-BayesOPT-Arxiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ICLR'21-BayesOPT-Arxiv/notation.tex <==
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\m}{\mathbf{m}}
\newcommand{\constraint}{\mathcal{C}}

==> ICLR'21-BayesOPT-Arxiv/sections/background.tex <==
\vspace{-.1in}
\section{Related Work}
\vspace{-.1in}

%This section describes prior work in the hardware and software optimizations for DNNs.

\subsection{Hardware to Optimize DNNs}
\vspace{-.1in}

Accelerators are specialized processors that provide significant performance
and efficiency improvements by targeting specific workloads; they also
typically require significant manual design.  For deep learning, these
primitives are often basic linear algebra subprograms (BLAS).

Prior work has designed specialized hardware to execute BLAS kernels.
Google's TPU~\citep{jouppi2017datacenter} uses large hardware structures
called systolic arrays~\citep{kung1979systolic}, and NVIDIA's GPUs have
tensor cores~\citep{v100}.  DianNao~\citep{chen2014diannao} computes fully
connected layers of a neural network using multiply-accumulate trees, and
its successor, DaDianNao~\citep{chen2014dadiannao}, improves data locality
for large neural networks by tiling processing elements (PEs) around on-chip
eDRAM banks.  A more specialized version, ShiDianNao~\citep{du2015shidiannao},
focuses on dense convolutional neural networks (CNNs), which exhibit regular
computational behavior with high data reuse.  Eyeriss~\citep{chen2016eyeriss}
and Eyeriss v2~\citep{chen2019eyeriss} also focus on CNNs, introducing
a specific dataflow that exploits a reuse pattern exhibited by 2D
convolutions.  To improve performance scaling, Eyeriss v2 uses a more
sophisticated interconnect than its predecessor, and it also introduces
a variant that targets sparse CNNs.  Prior work~\citep{parashar2017scnn,
zhang2016cambricon} has dealt with sparsity by suppressing zero-valued
activations and storing and operating on compressed data.  Many other
domain specific architectures have been proposed to take advantage
of local communication patterns~\citep{farabet2011neuflow}, 3D-stacked
bandwidth memory~\citep{kim2016neurocube, gao2017tetris}, or multi-chip
modules~\citep{shao2019simba}. Recent work~\citep{yang2020interstellar} presents heuristics for automatically
synthesizing hardware using a domain-specific language.

\vspace{-.1in}
\subsection{Software to Optimize DNNs}
\vspace{-.1in}

Software optimizations for reducing the compute and storage requirements
of neural networks include loop blocking (tiling), loop reordering, and
loop unrolling~\citep{whaley1998automatically, mullapudi2016automatically,
bondhugula2008practical}.  Compilers such as TVM~\citep{chen2018learning}
have used learned cost models to optimize execution efficiency.  Similarly,
Timeloop uses a grid or random search to optimize software mappings on a
user-specified hardware architecture~\citep{parashar2019timeloop}.  However,
all previous software optimizers treat hardware as a black box and ignore
interactions between hardware and software.

\ignore{
a black box without explicitly considering the interaction between hardware
and software, such as buffer sizing/utilization and parallelism usage.
}

Ours is the first work that systematically explores the space of both
hardware and software optimizations; this larger search space requires a
more principled search method, which motivates our constrained Bayesian
optimization framework.



==> ICLR'21-BayesOPT-Arxiv/sections/bayes_opt.tex <==

\vspace{-.175in}
\section{Bayesian Optimization}
\label{sec:bayesopt}
\vspace{-.125in}
\subsection{Overview}
\vspace{-.1in}

Bayesian optimization~\citep{jones1998efficient, brochu2010tutorial,
shahriari2015taking} is an effective approach for the optimization of
expensive, possibly noisy black-box functions.  BO has been used to 
optimize hyperparameters~\citep{snoek2012practical}, configure
algorithms~\citep{hutter2011sequential}, optimize A/B experiments
\citep{letham2019constrained}, and more.  For our problem, we have a
parameterized representation and access to a simulator. Since one of our
main concerns is sample efficiency, Bayesian optimization is particularly
suitable.

The actual cost of evaluation depends on the experimental infrastructure, but in general, it is much more expensive to evaluate a hardware design choice than to evaluate software optimizations, because hardware design can take hours (to produce a hardware simulator or an FPGA) to days or even months (to produce an ASIC).

% The actual cost of evaluation depends on the experimental infrastructure,
% but in general, the evaluation is much more expensive on hardware than
% software. For example, the evaluation of a hardware design choice requires
% a faithful hardware implementation and a search for the optimal software
% mappings, a process that can take hours (with a simulator or FPGA) to days
% or even months (for an ASIC).  By contrast, the cost of applying a list of
% software mappings and running the transformed workload is relatively low,
% ranging from seconds (in a simulator) to minutes (on a real hardware,
% FPGA or ASIC).

% In the remainder of this section, we provide a brief description of BO followed by its application to hardware/software co-design. In particular, we discuss our solution that covers both linear and non-linear constraints.

Bayesian optimization has two major components: (1) a surrogate model
provides a Bayesian posterior probability distribution that predicts
potential values of the objective function.  (2) an acquisition function
uses the model to identify the next point to evaluate.

% This provides a balance between exploration and exploitation, where exploration of high-uncertainty areas allows the search to find new promising regions of the parameter space, and exploitation finds the best parameters within a region.

\vspace{-.15in}
\subsection{Gaussian processes}
\vspace{-.1in}

A common surrogate model is a Gaussian process (GP)~\citep{gpml2006book} due to its simplicity and flexibility. A GP is prior distribution over the space of functions comprised of a mean function $m(\x)$ and a covariance, or kernel function $k(\x, \x')$. Suppose we are given a dataset of $N$ input/output pairs over a bounded domain $\Omega$ with $D$ input dimensions and scalar outputs. For brevity, we write this as $(X,\y)$, where $X \in \Omega^{N \times D}$ and $\y \in \mathbb{R}^N$. The posterior predictive distribution over function values $f$ for a new input $\x$ is given by $P(f \mid \x, X, \y) = \mathcal{N}(\mu(\x), \sigma^2(\x))$, where
\begin{align*}
    \mu(\x) &= K_{\x X} K_{XX}^{-1}(\y - \m_X) + m(\x), \\
    \sigma^2(\x) &= k(\x, \x) - K_{\x X}K_{XX}^{-1}K_{\x X}^\top.
\end{align*}
Where $K_{XX}$ is a matrix formed by evaluating the kernel on $X$, $K_{\x X}$ is the vector of kernel evaluations between $\x$ and $X$, and $\m_X$ is the vector of mean function evaluations on the input dataset.

A common choice for the kernel is squared exponential. Given two input vectors $\x_i$ and $\x_j$, this is defined as $k(\x_i, \x_j) = \alpha^2 \exp\left (-\frac{\|\x_i - \x_j\|^2}{\boldsymbol{\ell}^2}\right )$. $\alpha$ and $\boldsymbol{\ell}$ are kernel hyperparameters.
% $\alpha$ is the amplitude, which governs the range over which the function varies. $\boldsymbol{\ell}$ is a vector of lengthscales, which govern how quickly the function is likely to vary along each dimension.
% The inverse-lengthscales can be used as a measure of parameter importance. The squared exponential kernel places high prior density on smooth (infinitely differentiable) functions. We use this kernel when we do not have prior knowledge of the objective form, as will be the case for output constraints discussed later.

Another kernel that we find particularly useful is a linear kernel on top of explicit features. Given a feature mapping $\phi(\x): \mathbb{R}^D \rightarrow \mathbb{R}^K$, the linear kernel can be written as $k(\x_i, \x_j) = \phi(\x_i)^\top \phi(\x_j)$. When we have strong prior information about the relevant feature interactions that govern the black-box function, this kernel allows us to encode these interactions directly and produces a more sample-efficient posterior estimate.

In cases where the observations from the black-box function are noisy, we can add a noise kernel $K_\mathrm{noise} = \tau^2 \mathrm{I}$ to $K_{XX}$, where $\tau^2$ is a hyperparameter. This implies a Gaussian observation likelihood.

Following common practice, we use the constant mean $m(\x) = c \quad \forall \  \x$. All kernel and mean hyperparameters are learned by maximizing the marginal likelihood of the GP on the current dataset.

\vspace{-.1in}
\subsection{Acquisition functions}
\vspace{-.1in}

A critical component in the BO framework is the choice of acquisition function $a(\cdot)$ that assigns each design point a value that represents the utility of testing this point. Two commonly used acquisition functions are expected improvement (EI) and lower confidence bound (LCB).

EI computes the amount we expect to improve upon the current best observed objective value $y_* \equiv \mathrm{max}\{y_i\}_{i=1}^{N}$ by evaluating a design point $\x$. Formally, it can be written as
\begin{align*}
    a_{\mathrm{EI}}(\x) &= \int_{-\infty}^{\infty}\mathrm{max}(y_* - f, 0) P(f \mid \x, X, \y)\mathrm{d}f.
\end{align*}

\vspace{-.05in}
where $f$ is the latent function from the surrogate model, and $y_*$ is the best value observed.

% For each candidate point, we estimate this integral with 1000 samples from the posterior predictive distribution. There is a closed-form solution for EI, but with a sufficient number of samples there is little practical difference between the two forms.

LCB~\citep{srinivas2009gaussian} provides an explicit tradeoff between the predictive mean and variance and is defined as
\vspace{-.05in}
\begin{align*}
    a_\mathrm{LCB}(\x) &= \mu(\x) + \lambda \sigma(\x).
\end{align*}
Where $\lambda$ represents a tradeoff parameter. A small $\lambda$ promotes greater exploitation, and a large $\lambda$ promotes greater exploration. We found $\lambda=1$ to work well in our experiments. Beyond these, there are many other possible acquisition functions that could be used in future exploration~\citep{thompson1933likelihood, hennig2012entropy, hernandez2014predictive, frazier2009knowledge}.
\vspace{-.15in}
\subsection{Constraints}
\vspace{-.1in}

In our problem, the vast majority of the design space will produce invalid solutions.
% For software optimization, parameters are constrained by the available resources and shape given by the hardware. For hardware optimization, the parameters are constrained by e.g., the PE factors, local buffer sizes, and whether there is a valid, physically realizeable mapping.
When the constraints are a known function of the input features, we can directly account for them as input constraints. Otherwise, we must run the simulation and treat invalid points using an output constraint. Here, we will describe these constraint types, and how they are incorporated into BO.

% \vspace{-.1in}
\emph{Input constraints} are explicit constraints that are used when optimizing the acquisition function. They directly prevent the search from suggesting points that will violate the constraints. As some constraints are non-linear, this optimization is itself very challenging, as it is a global optimization problem with non-convex constraints. In the unconstrained case, maximizing the acquisition function often takes a hybrid approach: generating a random initial set of points and refining them by gradient ascent. Maintaining feasibility with non-convex constraints is far more challenging, however.

We therefore optimize the acquisition function in a simple way by performing rejection sampling on the design space: we randomly sample parameters until we obtain 150 feasible points, and then choose the one the maximizes the acquisition function. On average the sampling takes 22K random samples to get a pool of 150 feasible points. We have found that practically this is a simple yet effective strategy for our problems, we leave more involved optimization schemes for future work.

% \vspace{-.1in}
\emph{Output constraints} are used when we do not know the form of the constraint a-priori and must run the simulator to test feasibility. This is also referred to as an ``unknown'' constraint, and BO has been adapted to incorporate a constraint model in addition to the regression model~\citep{gelbart2014bayesian}. These simultaneously learn about the constraint boundaries while modeling the objective.

Let $\constraint(\x)$ denote the event that $\x$ satisfies constraint $\constraint$. Constrained BO uses a Bayesian classifier to model $P(\constraint(\x))$. It is relatively straightforward to adapt a GP regressor to 
classification~\citep{gpml2006book}.
% In our case, observations come in the form of binary observations, 1 if the observation is feasible and 0 otherwise. A GP models this by assuming a real valued function $f(\x)$ is drawn from a GP prior, which is then transformed through a link function (e.g., sigmoid or probit) to form a Bernoulli probability. Inference is no longer closed-form, but can be efficiently approximated through variational inference, expectation propagation, or Monte-carlo sampling \cite{gpml2006book}.

Under a Bayesian classifier, the acquisition function $a(\x)$ is modified to account for the probability that the constraint is satisfied, with 0 utility if it is not satisfied.
\begin{align*}
    \bar{a}(\x) &= \mathbb{E}[a(\x)\mathrm{I}[\constraint(\x)]] = P(\constraint(\x))a(\x).
\end{align*}
Where $\mathrm{I}[\constraint(\x)]$ is the indicator function that evaluates to 1 if the constraint is satisfied and 0 otherwise.
We therefore maintain two models: one regression model to capture the objective and one classifier to model the constraint in order to avoid evaluations in infeasible regions.


==> ICLR'21-BayesOPT-Arxiv/sections/conclusion.tex <==
\vspace{-.15in}
\section{Conclusion}
\label{sec:conclusion}
\vspace{-.1in}
% We cast hardware/software co-design as a bilevel bayesian optimization problem and demonstrate that out-of-the-box mechanisms have difficulty navigating the complex, constrained design space. We find that this is due to the unique constraints that hardware design entails and we propose a novel input/ouput constraint framework to allow the optimizer to effectively explore the space, enabling automatic search of new and efficient designs for a variety of model types. Using learning to automate hardware/software co-design opens up many opportunities beyond generating optimal hardware, notably transfer-learning, which would minimize design time across designs and models. The techniques we develop here are not limited to DNN accelerators, and while taping out custom chips for unique tasks may still be prohibitively expensive, as we enter the golden age of computer architecture~\cite{hennessy2019new}, developing automatic mechanisms for architectural exploring is critical to quickly and efficiently producing custom hardware architectures.

In this paper, we have cast hardware/software co-design as a Bayesian
optimization problem.  We have shown that standard mechanisms have
difficulty navigating the complex, highly constrained design space,
so we have presented a novel constrained formulation that
allows the optimizer to efficiently identify desirable points in this
design space.  The use of machine learning to automate hardware/software
co-design opens many opportunities for future work.  For example, transfer
learning could dramatically reduce design time across designs and models.
The techniques described here are not limited to DNN architectures,
which is significant because as we enter the golden age of computer
architecture~\citep{hennessy2019new}, it is essential that we develop
automatic mechanisms for architectural exploration that quickly produce
custom hardware accelerators.


% \newpage
% \section{Broader Impact of this Work}
% This paper provides three types of broader impact.  First, by improving
% the process of designing new energy-efficient DNN accelerators, it can reduce
% the carbon footprint of deep learning, which has been shown to comprise 1-2\%
% of global energy consumption~\cite{masanet2020recalibrating}.  Second,
% by automating much of the process of designing new DNN accelerators,
% our work democratizes the process of designing new DNN accelerators,
% allowing many more individuals to innovate.  Third, our work continues the
% trend of bringing together researchers from the machine learning community
% and the computer architecture community.

==> ICLR'21-BayesOPT-Arxiv/sections/evaluation.tex <==
\vspace{-.15in}
\section{Evaluation}
\vspace{-.1in}
\subsection{Methodology}
\vspace{-.1in}
\paragraph{Infrastructure} We conduct our evaluation on
Timeloop~\citep{parashar2019timeloop}, which is an open-source infrastructure
for evaluating the hardware design and software optimization of DNN
accelerators.  Timeloop represents the key architecture attributes of DNN
accelerators that realize a broad space of hardware structure and topology,
which generate an accurate projection of performance and energy efficiency
for DNN workloads.  In the evaluation, Timeloop takes two inputs: 1) the
hardware configuration, which consists of the hardware-related parameters,
and 2) the software mapping, which consists of the software parameters
that describe the mapping.  As most accelerators are designed for neural
network inference, we limit the use case to inference in this work and
leave training for future work.

\vspace{-.1in}
\paragraph{Workloads}  To show that our solution automatically produces efficient hardware for a variety of neural networks,
we use our BO framework to optimize critical layers from CNNs
(ResNet~\citep{he2016deep} and DQN~\citep{mnih2013playing}), as well as an
MLP and Transformer~\citep{vaswani2017attention}.

\vspace{-.1in}
\paragraph{Experimental Setup}  We use Eyeriss~\citep{chen2016eyeriss},
a state-of-the-art DNN accelerator, as our baseline.  All workloads are
evaluated on the Eyeriss implementation with 168 PEs~\citep{chen2016eyeriss}
except for the Transformer model, which runs on the larger version of Eyeriss
with 256 PEs~\citep{parashar2019timeloop}.  In the software mapping search,
we use Eyeriss's hardware specifications and search for the best software
mapping for each neural layer.  In the hardware search, we perform the search
under the same compute and storage resource constraints as Eyeriss for each
neural model.~\footnote{This work focuses on model-specific hardware, but
hardware specialization provides larger benefits at a finer granularity,
i.e. if different layers can execute on customized hardware. We leave
this for future work.} 
%This is possible when the hardware can be easily
% reconfigured (FPGAs), or when models are split among multiple accelerators
% (model parallelism).

\vspace{-.1in}
\paragraph{Metrics} Hardware accelerators are designed to achieve both speed
and energy efficiency, so we adopt the widely used energy-delay product
(EDP) as the objective.  Since EDP values can vary by an order of magnitude,
we normalize by dividing by the best (minimal) EDP value and take the
reciprocal for optimization curves.  For the hardware/software co-design, we
report the EDP improvements of each neural model, which is averaged across
all layers (see~Figure \ref{fig:cnn_layers} and \ref{fig:other_layers} in
the appendix).  For software mapping optimizations, we report the layer-wise
EDP improvements.

\vspace{-.1in}
\paragraph{Baselines} In hardware search, we compare against constrained random search that repeatedly takes the first random sample in the design space that satisfies the constraints.  In software search, we use constrained random search, TVM with XGBoost and TreeGRU~\citep{chen2018learning}, and out-of-the-box BO that optimizes in a continuous parameter space and rounds to the nearest valid parameters.

\vspace{-.1in}
\subsection{Software Mapping Optimization}
\vspace{-.1in}
We show the results of software mapping optimization first, as the
capability of finding a good mapping is the base of evaluating a hardware
design.  Figure~\ref{fig:sw_curves} shows the improvements of BO over
our constrained random search formulation.  Our BO formulation outperforms random search, both variants of TVM as well as a standard BO formulation that optimizes discrete parameters using a relax-and-round approach.
% This result is particularly interesting when compared to using BO for hyperparameter tuning, where out-of-the-box BO works much better in a less-constrained parameter space.

% \begin{figure}[h]
% \centering
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/sw/resnet-1.pdf}
%   \caption{ResNet-K1}
% \end{subfigure}
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/sw/resnet-2.pdf}
%   \caption{ResNet-K2}
% \end{subfigure}
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/sw/resnet-3.pdf}
%   \caption{ResNet-K3}
% \end{subfigure}
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/sw/resnet-4.pdf}
%   \caption{ResNet-K4}
% \end{subfigure}
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/sw/dqn-1.pdf}
%   \caption{DQN-K1}
% \end{subfigure}
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/sw/dqn-2.pdf}
%   \caption{DQN-K2}
% \end{subfigure}
% \caption{Software mapping optimization on ResNet and DQN. The Y-axis shows the reciprocal of energy-delay product (EDP). Higher is better.}
% \label{fig:sw_cnn}
% \end{figure}

% \begin{figure}[h]
% \centering
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/sw/mlp-1.pdf}
%   \caption{MLP-K1}
% \end{subfigure}
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/sw/mlp-2.pdf}
%   \caption{MLP-K1 \kevin{I'm guessing this is supposed to be K2?}}
% \end{subfigure}
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/sw/transformer-1.pdf}
%   \caption{Transformer-K1}
% \end{subfigure}
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/sw/transformer-2.pdf}
%   \caption{Transformer-K2}
% \end{subfigure}
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/sw/transformer-3.pdf}
%   \caption{Transformer-K3}
% \end{subfigure}
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/sw/transformer-4.pdf}
%   \caption{Transformer-K4}
% \end{subfigure}
% \caption{Software mapping optimization on Transformer and MLP. The y-axis shows the reciprocal of energy-delay product (EDP). Higher is better.}
% \label{fig:sw_others}
% \end{figure}

\begin{figure}[h]
\centering
\vspace{-.1in}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\textwidth]{figures/appendix/resnet-2.pdf}
  \caption{ResNet-K2}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\textwidth]{figures/appendix/dqn-2.pdf}
  \caption{DQN-K2}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\textwidth]{figures/appendix/mlp-2.pdf}
  \caption{MLP-K2}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\textwidth]{figures/appendix/transformer-2.pdf}
  \caption{Transformer-K2}
\end{subfigure}
\caption{Software mapping optimization on layer 2 of ResNet, DQN, MLP, and Transformer. The y-axis shows the reciprocal of energy-delay product (EDP) (normalized against the best EDP value). Higher is better. Results for other layers can be found in the appendix. Best viewed in color.}
\vspace{-.2in}
\label{fig:sw_curves}
\end{figure}


\subsection{Hardware Configuration Optimization}
\vspace{-.1in}
%The evaluation of hardware search also involves the search of the software mapping. 
Figure~\ref{fig:hw_curves} shows the optimization curves for hardware/software co-design. The comparison of hardware search algorithms shows that BO provides consistently better performance than the constrained random search, and the comparison of software search algorithms shows the importance of mapping optimization in the co-design process. As shown in Figure~\ref{fig:hw_compare}, we find that the designs searched by BO achieve significantly better EDP on all neural models compared to the state-of-the-art manually designed accelerator (18.3\%, 40.2\%, 21.8\% and 16.0\% for ResNet, DQN, MLP and Transformer respectively).

\begin{figure}[ht]
\centering
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\textwidth]{figures/hw/hw_curve_resnet.pdf}
  \caption{ResNet}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\textwidth]{figures/hw/hw_curve_dqn.pdf}
  \caption{DQN}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\textwidth]{figures/hw/hw_curve_mlp.pdf}
  \caption{MLP}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=1\textwidth]{figures/hw/hw_curve_transformer.pdf}
  \caption{Transformer}
\end{subfigure}
\caption{Hardware/software co-optimization. The x-axis shows the number of trials for hardware search, and 250 attempts are made to find the optimal software mapping for each layer in the model on the hardware specification. Best viewed in color.}
\vspace{-.2in}
\label{fig:hw_curves}
\end{figure}


% \begin{wrapfigure}[20]{r}{0.5\textwidth}
%   \centering
%   %\includegraphics[width=0.2\textwidth]{figures/assembly.pdf}
%   \includegraphics[width=0.5\textwidth]{figures/hw/hw_bars.pdf}
%   \caption{Comparison between the SOTA accelerator (Eyeriss) and searched design. Results are EDPs normalized to Eyeriss, and lower is better.}  \label{fig:graph}
% \end{wrapfigure}\leavevmode

\vspace{-.05in}
\subsection{Ablation Studies}
\vspace{-.1in}
\paragraph{Surrogate models and acquisition functions}  There exist
popular variants for both the surrogate models and acquisition functions.
In Figure~\ref{fig:bo_ablation}, we compare the surrogate models of Gaussian
process (GP) with random forest (RF) and the acquisition functions of
expected improvement (EI) and lower confidence bound (LCB).  As shown,
in the transformed feature space, GP generally performs better than RF,
and LCB generally outperforms EI.

% \begin{figure}[ht]
% \centering
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/ablation_acquisition/gp-2.pdf}
%   \caption{ResNet-K2}
% \end{subfigure}
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/ablation_acquisition/gp-3.pdf}
%   \caption{ResNet-K3}
% \end{subfigure}
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/ablation_acquisition/gp-4.pdf}
%   \caption{ResNet-K4}
% \end{subfigure}
% \caption{GP with different surrogate models and acquisition functions.}
% \label{fig:sw_ablation_gp}
% \end{figure}

\paragraph{Exploration vs. Exploitation} The LCB acquisition function explicitly balances exploration and exploitation with a hyperparameter ${\lambda}$. To further study the impact of exploration vs. exploitation in the use of LCB, we test LCB with different ${\lambda}$ values in Figure~\ref{fig:lcb_ablation}. We find that LCBs with ${\lambda}$ values that are greater than 0.5 provide stable performance in the optimization curves, while LCB with ${\lambda}=0.1$ suffers from insufficient exploration.

\begin{figure}[ht]
\centering
\vspace{-.1in}
\begin{subfigure}{0.33\textwidth}
  \includegraphics[width=1\textwidth]{figures/hw/hw_bars.pdf}
  \caption{Comparison with Eyeriss.}
  \label{fig:hw_compare}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
  \centering
  \includegraphics[width=1\textwidth]{figures/ablation_acquisition/gp-4.pdf}
  \caption{BO ablation}
  \label{fig:bo_ablation}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\textwidth]{figures/ablation_acquisition/lcb-4.pdf}
  \caption{LCB $\lambda$ ablation}
  \label{fig:lcb_ablation}
\end{subfigure}
\caption{(\subref{fig:hw_compare}): Comparison between the SOTA accelerator (Eyeriss) and searched design. Results are EDPs normalized to Eyeriss, and lower is better. (\subref{fig:bo_ablation})-(\subref{fig:lcb_ablation}): Ablation studies on ResNet-K4. Higher results are better. (\subref{fig:bo_ablation}) BO with different surrogate models and acquisition functions. (\subref{fig:lcb_ablation}) LCB acquisition function with different $\lambda$ values.}
\vspace{-.25in}
\label{fig:ablations_and_hwcompare}
\end{figure}

% \begin{figure}[ht]
% \centering
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/ablation_acquisition/lcb-2.pdf}
%   \caption{ResNet-K2}
% \end{subfigure}
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/ablation_acquisition/lcb-3.pdf}
%   \caption{ResNet-K3}
% \end{subfigure}
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=1\textwidth]{figures/ablation_acquisition/lcb-4.pdf}
%   \caption{ResNet-K4}
% \end{subfigure}
% \caption{LCB acquisition function with different lambda values.}
% \label{fig:sw_ablation_lcb}
% \end{figure}


\vspace{-.05in}
\subsection{Architectural Insights}
\vspace{-.1in}
To show that our automated design can produce new architectural insights,
we provide a qualitative comparison of Eyeriss with our solution for DQN.
Our design predominantly differs in the shape of the PE array, as well
as in the number of memory buffers used.  Eyeriss allocates the majority
of its local buffer storage for filter weights, which are poorly utilized.
Our design increases buffer utilization by storing multiple inputs and
output elements.

\ignore{
One of the benefits of automated design is the opportunity to gain new
architectural insights. To demonstrate this, we provide a qualitative
comparison of Eyeriss with our solution for DQN. Our design predominantly
differs in the shape of the PE array, as well as how memory buffers are
allocated. Eyeriss allocates the majority of its local buffer storage for
filter weights, but it is poorly utilized. Our design increases buffer
utilization by storing multiple inputs and output elements as well.
}

We can also plug our hardware configuration into the heuristic-based
optimizer from prior work \citep{parashar2019timeloop} and attempt to
find a software mapping.  We do this using the 12$\times$14 PE array from
DQN.  Timeloop's software optimizers are unable to find the same mapping
that we do, with the best result being 52\% worse than the baseline.
This demonstrates the utility of a learned co-design approach that enables
the software optimizer to be robust across different hardware architectures.


%Interestingly,  heuristic-based optimizers find our solution sub-optimal and worse than Eyeriss. Compared to Eyeriss's 14$\times$12 PE array, our design adopts the 12$\times$14 PE array structure. Timeloop's software optimizers (both grid search and random search) show that 12$\times$14 is 52\% worse than 14$\times$12, as they fail to find the optimal mapping on the 12$\times$14 architecture. This shows that heuristic-based software optimizers are often hardware dependent, thus are unsuitable in the co-design approach that requires the software optimizer to be robust across different hardware architectures. 


==> ICLR'21-BayesOPT-Arxiv/sections/formulation.tex <==
\vspace{-.1in}
\section{Bayesian Optimization for Hardware/Software Co-design}
\vspace{-.1in}
% \begin{figure}[ht]
% %    \begin{subfigure}{.55\textwidth}
% %      \centering
% %      \includegraphics[width=1\textwidth]{figures/overview_new.pdf}
% %    \end{subfigure}
% %    \begin{subfigure}{.45\textwidth}
% %      \centering
% %      \includegraphics[width=1\textwidth]{figures/code_new.pdf}
% %    \end{subfigure}
% \centering
% \includegraphics[width=1\textwidth]{figures/overview.pdf}
% \caption{Overview of BO-based nested search for hardware/software co-design.}
% \vspace{-.2in}
% \label{fig:model}
% \end{figure}

\subsection{Overview of Nested Hardware/Software Optimization}
\vspace{-.1in}
Provided the constraints discussed in Section \ref{sec:hwsw_representation} and the BO formulation from Section \ref{sec:bayesopt}, we propose a nested approach for co-optimizing hardware/software parameters. The overall approach is outlined in Figure~\ref{fig:model}. The goal is to find the optimal hardware parameters for a neural model and the optimal set of software parameters for each layer in the neural model. Since software constraints depend on a feasible hardware design, we first propose the hardware parameters, then for that hardware co-optimize the software mapping. 

Specifically, let $\x_h$ and $\x_s$ denote the set of hardware and software parameters in the parameter space to be optimized. In the nested search process, we first use the hardware optimizer to generate a design of hardware. In particular, we perform the hardware search in the space of possible hardware $\mathcal{S}_h$ to optimize all hardware parameters, where the objective is to minimize $f(\x_h \mid \textrm{NN})$ which we define as the energy-delay product (EDP) of running the neural network (NN) model on the given hardware, assuming the optimal software mapping for each individual layer. This step produces a hardware specification and can be formalized as $\textrm{{argmin}}_{h\in\mathcal{S}_h} f(\x_h \mid \textrm{NN})$.

For the chosen hardware design, our framework performs the software search for each individual neural layer in its constrained software mapping space $\mathcal{S}_s|h, \textrm{NN}_j$ to optimize the mapping parameters, where $\textrm{NN}_j$ denotes the $j$th layer in the neural network model, and the objective becomes $f(\x_s \mid \x_h, \textrm{NN}_j)$, which is defined as the EDP of running the layer $j$ on the fixed hardware. This step produces a design point that represents the best set of software mappings for each layers on the given hardware structure, and can be formalized as $\textrm{{argmin}}_{s\in\mathcal{S}_s|h} f(\x_s \mid \x_h)$. The layerwise EDPs are then summed up as the EDP of the neural model, which is fed back to the hardware optimizer to generate the next hardware setting.

The iterative search between hardware and software will repeat for a user-defined number of trials. In this work, we set 50 for hardware search and 250 for software search. The combination of hardware and software that achieves the best EDP during the optimization process becomes the final model-specific hardware structure and layer-specific software mappings. A random sample is used in the first iteration of both the hardware and software search. In our Bayesian optimization (BO) framework, we use separate BO models to search in the hardware and software space. We now describe their design considerations, particularly the choice of kernel and feature transformation.
\vspace{-.1in}
\subsection{BO for Optimizing Hardware Architectures}
\vspace{-.1in}
\paragraph{Kernel design} The main design choice for BO is the GP kernel to use. For the hardware search, we choose a linear kernel on top of feature transformations that represent the relationship between the different parameters. This feature transformation allows us to explicitly encode domain knowledge. For example, by comparing the layout parameters of the 2D PE array and global buffer we can obtain the ratio between these adjacent storage layers, which correlates to the maximal degree of parallel buffer accesses in each dimension. The details of the features are given Figure~\ref{fig:features} in the appendix. We also add a noise kernel to deal with noise in the hardware evaluation. This is because the software optimizer is not guaranteed to find the best software mapping for each layer. There is some randomness in the software search, and therefore independent runs of software optimization for a fixed hardware design may yield different results.

\vspace{-.1in}
\paragraph{Constraints} There are both known and unknown constraints in the hardware search. The known constraints, such as the compute and storage budget, are treated as input constraints that reject invalid samples. The unknown constraints have to do with feasibility (if there exist valid software mappings of neural layers onto the hardware, and if the valid mappings can be sampled during the software optimization). Following Section~\ref{sec:bayesopt}, these constraints are treated as output constraints and are modeled by a GP with a squared exponential kernel. 
\vspace{-.1in}
\subsection{BO for Optimizing Software Mappings}
\vspace{-.1in}
\paragraph{Kernel design} Similar to hardware optimization, we use a linear kernel and transform the parameters to features that encode relational information. As the hardware is fixed in the search of software mappings, we are able to compute features such as buffer usage, which potentially help make the predictions more accurate. The evaluation of a mapping on a given hardware is deterministic in our infrastructure, thus there is no need for a noise kernel in the GPs.

\vspace{-.1in}
\paragraph{Constraints} As both the hardware and neural model are known during software optimization, all constraints are known and are treated as input constraints that automatically reject invalid samples.

%\subsection{Hardware Optimization with BO}
%A fixed hardware design choice presents a space of possible transformations that can be applied on the computation, including tiling, permutation and parallelism. Let $x_S$ denote the set of parameters that represents the software transformation. which consist of tiling parameters $X_{T}$ and permutation parameters $X_{P}$. Note that given the hardware design, parallelism is implicitly defined by a subset of tiling parameters and permutation parameters. The goal of this paper is to minimize $f(x_S)$, which is energy consumption on the given hardware.

%%subsection{SW Optimization with BO}
%The main characteristic is that, once the hardware design is fixed, the software optimization comes with a series of constraints, both linear and non-linear. In particular, the constraints come from the fact that the tiling parameters need to be consistent with the workload, and that the data cannot exceed the buffer capacity at each storage layer, and that resources required by parallel computation cannot exceeds available hardware instances.

% \subsection{Hardware Parameters and Constraints}
% As discussed, we search for the optimal resource configurations and dataflow configurations. As shown in Figure~\ref{fig:hw_params}, the resource parameters include the X-Y dimensional layout of 2D the PE array, the local buffer partition and the global buffer organization and specification. The dataflow parameters determine the partial usage of PEs that are implemented in hardware.

% The hardware constraints mainly come from the total amount of PEs and buffer resources. The main "unknown" constraint is that if the hardware configuration allows any valid software mapping. For example, if the buffer size is not enough for a specific type of data (inputs, weights or outputs), it is possible that no valid mapping can be found or sampled in the limited trials. Figure~\ref{fig:hw_cons} lists the hardware constraints.

% \subsection{Software Parameters and Constraints}
% Once the hardware is fixed, it exposes a set of parameters and constraints to the software optimizer. In particular, the parameters include the blocking factors that decide the usage of each level of memory hierarchy and degree of parallelism, and loop orders that determine the reuse patterns at each level of memory. Figure~\ref{fig:sw_params} describe a list of parameters in detail.

% The software mapping optimization are constrained by both the hardware resources and shapes of neural networks. On the hardware side, the mapping is limited by the amount of hardware resources, including buffer size and number of PEs in each of the 2D dimension that can be utilized in parallel. On the other hand, the shape of neural networks along each shape dimension determines the possible factors and its combinations across layers of storage. More details can be found in Figure~\ref{fig:sw_cons}.

==> ICLR'21-BayesOPT-Arxiv/sections/hwsw_representation.tex <==
\vspace{-.2in}
\section{A Formal Representation of Software and Hardware}
\label{sec:hwsw_representation}
\vspace{-.1in}

Hardware/software co-design typically performed manually, but we believe that
this vast design space is best navigated by an intelligent search process.
To facilitate this automation, this section formally defines the hardware
and software design spaces.

% Both hardware and software exhibit large design spaces, and it is often
% difficult to efficiently characterize one without the other. The process
% that computer architects take to develop new primitives for hardware based
% on software is often referred to as hardware/software co-design. This is
% often a manual process, with architects leveraging heuristics, constraints,
% and intuition to guide the search. In this section, we parameterize both
% the hardware and software design spaces such that a learning algorithm
% can automatically explore and optimize them.

\vspace{-.15in}
\subsection{Parameterizing the Design Space}
\vspace{-.1in}

\textit{Software design points} can be parameterized by the loop ordering, loop
tiling, and computational parallelism of the seven-level loop nest used to
compute a convolutional layer (see appendix), as has been
noted by recent work~\citep{parashar2019timeloop, yang2020interstellar}. These
software parameters are subject to hardware constraints, such as the quantity
and layout of processing elements (PEs) and the size of storage elements.

\textit{Hardware parameters} \ignore{are generally more specific to the
low-level resource and memory configurations or the layout of PEs.  These}
can be broken down into a two broad categories:

\textit{Resource configurations} represent the
physical aspects of hardware, such as buffer sizes, tile sizes, and the
cluster size of global buffers, as well as the layouts of the PE array
and of the global buffer.

\textit{Dataflow configurations} represent the usage
of the PE array that are implemented in hardware, such as the blocking
factors and degree of parallelism at the PE level, which also determines
the communication patterns among PEs.

Figure~\ref{fig:conv1d} shows two possible design points for a 1D
convolution.  Both design points tile and parallelize the channel (C)
dimension.  To the right of each component in the architecture is a set of
loops that specifies the control logic for the component, which can be broken
down into temporal streaming (\texttt{for} loops) and spatial distribution
(\texttt{parallel\_for} loops).  For example, in the architecture on the
left, the global buffer distributes across the PEs 1 weight from 4 separate
channels (\texttt{c2}), and the PEs perform all operations that the weight
participates in.  In this design, all data reuse is captured within the PE,
so the global buffer need not store anything.  By contrast, the architecture
on the right distributes a single output element across the PEs to compute
partial sums, which are stored in the global buffer across iterations.
Both these design points consist of the same architectural components,
but the dataflows vary, imposing different constraints on the software.
The appendix shows the details of the parameterization of a more practical
2D convolution.

\vspace{-.15in}
\begin{figure}[ht]
  \centering
  \includegraphics[width=\textwidth]{figures/examples/conv1d.pdf}
  \caption{Two architectures computing a 1D convolution.}
  \label{fig:conv1d}
  \vspace{-.1in}
\end{figure}

\vspace{-.1in}
\subsection{Constraints in the Design Space}
\vspace{-.1in}

There are several reasons why the vast space of hardware and software
parameters is filled with impractical or invalid design points.
First, hardware designs are fundamentally constrained by area (the total
amount of compute and storage resources) and factors such as available
memory bandwidth.  Second, the design cost and latency of additional area
grow super-linearly~\citep{shao2019simba}, which leads to many impractical
design points.

Software constraints are generally governed by feasibility instead of
practicality and predominantly depend on the hardware configuration and the
specific neural network workload.  For a specific hardware accelerator, there
is a limited number of available resources, so the software optimization
problem can be viewed as a search for the most efficient use of hardware
PEs and buffers.  For example, the loop blocking optimization factors a
neural network across multiple hardware storage buffers---and the feasible
factorizations are constrained by the size of the hardware buffers.

%\subsection{Terminology}
%This work uses machine learning both as a optimization tool and as targets. Some terms, such as \textit{models} and \textit{parameters} can be interpreted differently in different contexts. To avoid confusion, here we clarify the use of terminology. We refer to deep neural networks (DNNs) as \textit{DNN workload}, which are the models that this paper is optimizing for. Bayesian Optimization (BO) is referred as is, which consist of a surrogate model and acquisition function. BO explores the \textit{search space} of both hardware and software to find optimal \textit{design choices/points}. Each design choice/point consists of a list of \textit{parameters} and each parameter can take on different \textit{values}.


==> ICLR'21-BayesOPT-Arxiv/sections/introduction.tex <==
\section{Introduction}
\vspace{-.1in}

The compute requirements of deep learning are growing at a double
exponential rate~\citep{hern2020measuring}, with more powerful
models requiring exponentially more compute to train.  This growth has been
enabled by large systems of hardware accelerators, like GPUs and
TPUs~\citep{v100, jouppi2017datacenter}.  However, the continued scaling of
these systems is limited by issues of power density, cooling, and memory, so we need to improve computational efficiency.

Efficiency improvements can be sought at each layer of the deep learning
stack, from better learning algorithms~\citep{kingma2014adam}, to improved
neural network architectures~\citep{tan2019efficientnet}, to deep learning
compilers~\citep{chen2018learning}, to specialized DNN accelerators that
increase hardware efficiency~\citep{chen2014diannao, chen2016eyeriss}.
In this paper, we focus on the low-level software and hardware portions
of this stack, with the goal of automatically optimizing the $energy\times
delay$ product of executing a particular model on a hardware accelerator.
We consider two components from the deep learning stack:  the hardware
accelerator and the software compiler that maps a model onto that hardware.
This area is commonly referred to as hardware/software co-design, and since
it requires human expertise from multiple disciplines (software engineers,
compiler writers, hardware architects), it is typically driven by manual
heuristics or heuristic-based search~\citep{yang2020interstellar}.

We propose a different approach, recognizing that for a given DNN model,
this hardware/software co-design can be framed as a joint search of the
space of all of the valid mappings and hardware architectures that can
correctly execute the model.  We formally parameterize this space based
on prior work~\citep{parashar2019timeloop}, and we find that standard
optimization techniques, including off-the-shelf Bayesian optimization,
perform poorly because the design space is semi-discrete and the vast majority of the
points in the space are infeasible. Prior work~\citep{nardi2019practical} makes a similar observation, noting that (1) complex constraints such as hardware area and energy budget limit the feasible parameter values (i.e. small feasibility set), (2) some constraints are unknown until after a sample point has been evaluated (i.e. unknown feasibility).

% the set of feasible hardware designs is vast and highly sparse.

Our solution casts the search as a bilevel optimization problem, as shown in Figure \ref{fig:model}.  The outer
loop optimizes over hardware architectures, while the inner loop optimizes
over software mappings for a given architecture.  Both of these are heavily
constrained black-box global optimization problems that require expensive
simulations to obtain performance estimates.  We therefore propose a nested,
constrained Bayesian optimization (BO) formulation that uses Bayesian
models of hardware and software performance to guide the search towards
promising regions of the design space.  Our approach is extensible to a
variety of different neural network architectures, and we make the code
publicly available.

% We therefore propose a a bilevel constrained Bayesian optimization (BO)
% algorithm.  To co-design the hardware and software layers, we employ an
% iterative approach that alternately optimizes the hardware architecture
% and the software mapping for that architecture.  Our optimization approach
% is extensible to a variety of different neural network architectures,
% and we make the code available for future investigation.

We find that when compared against the state-of-the-art manually-designed
hardware accelerators that use heuristic software mappings, our BO-based
approach provides significant improvements in the speed and energy efficiency
of the resulting system, improving the energy-delay product (EDP) by 16.0\%
to 40.2\% on a series of neural networks.  The key to our solution is
our robust BO software optimizer, whose consistent efficiency allows our
approach to scale to this huge search space.

This paper makes the following contributions:
\vspace{-.1in}
\begin{itemize}
    \item We present the first system that automatically co-optimizes both the hardware and software portions of DNN accelerator design using a principled and systematic search algorithm.

    \item We present a constrained formulation of hardware and software design for BO, a challenging problem given the high ratio (90\%) of invalid hardware and software designs.

    \item We present a nested hardware/software formulation of BO that is extensible to other hardware accelerator designs.

    \item We provide model-specific hardware and state-of-the-art results on multiple
          models.
\end{itemize}

\begin{figure}[t]
%    \begin{subfigure}{.55\textwidth}
%      \centering
%      \includegraphics[width=1\textwidth]{figures/overview_new.pdf}
%    \end{subfigure}
%    \begin{subfigure}{.45\textwidth}
%      \centering
%      \includegraphics[width=1\textwidth]{figures/code_new.pdf}
%    \end{subfigure}
\centering
\includegraphics[width=1\textwidth]{figures/overview.pdf}
\caption{Overview of BO-based nested search for hardware/software co-design.}
\vspace{-.2in}
\label{fig:model}
\end{figure}


==> ICLR'21-BayesOPT-Arxiv/sections/solution_software.tex <==
\section{Software Optimization with BO}
We propose a Bayesian Optimization (BO) framework to search for an optimal software transformation. We begin with a brief description of Bayesian optimization followed by its application to software transformation optimization. In particular, we discuss our solution to deal with both linear and non-linear constraints. 

\subsection{Bayesian Optimization}
Bayesian Optimization (BO) is a black box optimization method particularly suitable for problems with low dimension and expensive evaluation. Bayesian Optimization has two two main components: a Bayesian surrogate model and an acquisition function. The surrogate model provides a Bayesian posterior probability distribution that predicts potential values for the objective function. The most commonly used surrogate model for Bayesian optimization are Gaussian processes (GPs). We model the objective function $f$ using a GP with prior distribution $\mathcal{N}(\mu_0, \Sigma_0)$ where $\mu_0$ is a constant mean function and $\Sigma_0$ is covariance matrix with Matern Kernel, which are defined as follow~\zhan{still working on this with Kevin, to be filled.}:

The second major component is the acquisition function $\mathcal{A}$ that assigns each design point a value that represents the utility of testing this point. Among a few popular choices, we use expected improvement (EI) as the acquisition function, which is defined as:

\begin{equation}
    \textrm{EI}_n(x) = \mathop{\mathbb{E}}[\textrm{max}(h(x_S) - h_n^{*}, 0)]
\end{equation}

where $h$ is the surrogate model, and $h_n^{*}$ is the best value observed.

\subsection{Parameters and Constraints}
\paragraph{Parameters} We aim to search for a list of parameters $x_S$ that represent a near-optimal software transformation. The parameters are tiling parameters $x_{T}$ and permutation parameters $x_{P}$. More specifically, as shown in Table~\ref{fig:parameter}, given the hardware being Eyeriss~\citep{chen2016eyeriss}, there are 17 tiling parameters that factorize the workload along 6 dimensions in CNN computation (weight width, weight height, input width, input height, input channel, output channel), and 5 permutation parameters for the storage layers (register file, global buffer and DRAM). To ensure that the parameters take on the valid values, they are treated by a relax-and-round approach. In particular, a group of tiling parameters belong to same dimension (e.g. input channel) are rounded together to make sure they meet the dimension constraints (see next paragraph). 

\paragraph{Constraints} The hardware and workload imposes hard constraints in the software transformation optimization. Coming from the hardware side, the capacity of each storage layer is fixed, which limits the possible values of tiling parameters, which we refer to as \textit{capacity constraints}. In addition, resources required by parallel computation cannot exceeds available hardware instances, which we refer to as \textit{parallelism constraints}. Coming from the workload, the product of all tiling parameters along each dimension need to be equal to the corresponding dimension in the workload, which is referred to as \textit{dimension constraints}. Table~\ref{fig:constraints} lists all the constraints when optimizing a ResNet~\citep{he2016deep} layer on Eyeriss. As shown, all constraints are non-linear, including equality and inequality, which makes the optimization problem challenging.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/parameters.pdf}
  \caption{Parameters.}
  \label{fig:parameter}
\end{figure}

\subsection{Dealing with Constraints in BO}
\paragraph{Linearize Multiplicative Constraints.} For the constraints are in the form of pure multiplication, they can be converted into linear constraints and then treated as input constraints in BO. The conversion is realized with the logarithm trick. For example, instead of optimizing $x_9$, $x_{10}$, $x_{11}$ that have to meet the constraint $x_9 * x_{10} * x_{11} = 128$, we can optimize $log(x_9)$, $log(x_{10})$, $log(x_{11})$ with the constraint $log(x_9) + log(x_{10}) + log(x_{11}) = 7$. In this way, we can linearize all multiplicative constraints and specify them as input constraints.

\paragraph{Separate Classifiers for Non-Linear Constraints.} After linearizing the multiplicative constraints, the constraints that are originally affine becomes non-linear, and the constraints that are originally a mixture of affinity and multiplication remain non-linear. To deal with those non-linear constraints, we treat each of them as a separate output constraint, and use a separate GP that outputs a feasibility, which is the probability of the constraint being met. \footnote{Some input constraints are also specified as output constraints because the input constraints are not always satisfied.} We then combine the output constraints into the objective using \textit{feasibility-weighted objective}, which multiply the original EI value with the feasibility for all constraints as follows: 

\begin{equation}
    {Constrained}{EI} = EI * \prod_{i} P_i
\end{equation}

where $P_i$ is the probability of the $i$th constraint being met. This means the acquisition function is a composition of the different GPs. Moreover, since all of the constraints are known and each constraint is dealt with by a different classifier on their respective data, we expand each all terms to make it a linear constraint and use a linear kernel in all constraint GPs, which requires less training data.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/constraints.pdf}
  \caption{Constraints.}
  \label{fig:constraints}
\end{figure}

==> sections/solution_software.tex <==
\section{Software Optimization with BO}
We propose a Bayesian Optimization (BO) framework to search for an optimal software transformation. We begin with a brief description of Bayesian optimization followed by its application to software transformation optimization. In particular, we discuss our solution to deal with both linear and non-linear constraints. 

\subsection{Bayesian Optimization}
Bayesian Optimization (BO) is a black box optimization method particularly suitable for problems with low dimension and expensive evaluation. Bayesian Optimization has two two main components: a Bayesian surrogate model and an acquisition function. The surrogate model provides a Bayesian posterior probability distribution that predicts potential values for the objective function. The most commonly used surrogate model for Bayesian optimization are Gaussian processes (GPs). We model the objective function $f$ using a GP with prior distribution $\mathcal{N}(\mu_0, \Sigma_0)$ where $\mu_0$ is a constant mean function and $\Sigma_0$ is covariance matrix with Matern Kernel, which are defined as follow~\zhan{still working on this with Kevin, to be filled.}:

The second major component is the acquisition function $\mathcal{A}$ that assigns each design point a value that represents the utility of testing this point. Among a few popular choices, we use expected improvement (EI) as the acquisition function, which is defined as:

\begin{equation}
    \textrm{EI}_n(x) = \mathop{\mathbb{E}}[\textrm{max}(h(x_S) - h_n^{*}, 0)]
\end{equation}

where $h$ is the surrogate model, and $h_n^{*}$ is the best value observed.

\subsection{Parameters and Constraints}
\paragraph{Parameters} We aim to search for a list of parameters $x_S$ that represent a near-optimal software transformation. The parameters are tiling parameters $x_{T}$ and permutation parameters $x_{P}$. More specifically, as shown in Table~\ref{fig:parameter}, given the hardware being Eyeriss~\citep{chen2016eyeriss}, there are 17 tiling parameters that factorize the workload along 6 dimensions in CNN computation (weight width, weight height, input width, input height, input channel, output channel), and 5 permutation parameters for the storage layers (register file, global buffer and DRAM). To ensure that the parameters take on the valid values, they are treated by a relax-and-round approach. In particular, a group of tiling parameters belong to same dimension (e.g. input channel) are rounded together to make sure they meet the dimension constraints (see next paragraph). 

\paragraph{Constraints} The hardware and workload imposes hard constraints in the software transformation optimization. Coming from the hardware side, the capacity of each storage layer is fixed, which limits the possible values of tiling parameters, which we refer to as \textit{capacity constraints}. In addition, resources required by parallel computation cannot exceeds available hardware instances, which we refer to as \textit{parallelism constraints}. Coming from the workload, the product of all tiling parameters along each dimension need to be equal to the corresponding dimension in the workload, which is referred to as \textit{dimension constraints}. Table~\ref{fig:constraints} lists all the constraints when optimizing a ResNet~\citep{he2016deep} layer on Eyeriss. As shown, all constraints are non-linear, including equality and inequality, which makes the optimization problem challenging.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/parameters.pdf}
  \caption{Parameters.}
  \label{fig:parameter}
\end{figure}

\subsection{Dealing with Constraints in BO}
\paragraph{Linearize Multiplicative Constraints.} For the constraints are in the form of pure multiplication, they can be converted into linear constraints and then treated as input constraints in BO. The conversion is realized with the logarithm trick. For example, instead of optimizing $x_9$, $x_{10}$, $x_{11}$ that have to meet the constraint $x_9 * x_{10} * x_{11} = 128$, we can optimize $log(x_9)$, $log(x_{10})$, $log(x_{11})$ with the constraint $log(x_9) + log(x_{10}) + log(x_{11}) = 7$. In this way, we can linearize all multiplicative constraints and specify them as input constraints.

\paragraph{Separate Classifiers for Non-Linear Constraints.} After linearizing the multiplicative constraints, the constraints that are originally affine becomes non-linear, and the constraints that are originally a mixture of affinity and multiplication remain non-linear. To deal with those non-linear constraints, we treat each of them as a separate output constraint, and use a separate GP that outputs a feasibility, which is the probability of the constraint being met. \footnote{Some input constraints are also specified as output constraints because the input constraints are not always satisfied.} We then combine the output constraints into the objective using \textit{feasibility-weighted objective}, which multiply the original EI value with the feasibility for all constraints as follows: 

\begin{equation}
    {Constrained}{EI} = EI * \prod_{i} P_i
\end{equation}

where $P_i$ is the probability of the $i$th constraint being met. This means the acquisition function is a composition of the different GPs. Moreover, since all of the constraints are known and each constraint is dealt with by a different classifier on their respective data, we expand each all terms to make it a linear constraint and use a linear kernel in all constraint GPs, which requires less training data.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.8\textwidth]{figures/constraints.pdf}
  \caption{Constraints.}
  \label{fig:constraints}
\end{figure}
